Comprehensive models of novae at metallicity $Z = 0.02$ and $Z = 10^{-4}$

Novae are the observational manifestations of thermonuclear runaways on the surface of accreting white dwarfs (WDs). Although novae are an ubiquitous phenomenon, their properties at low metallicity are not well understood. Using the publicly-available stellar evolution code Modules for Experiments in Stellar Astrophysics (MESA), we model the evolution of accreting carbon-oxygen WDs and consider models which accrete matter with metallicity Z=0.02 or $10^{-4}$. We consider both models without mixing and with matter enriched by CO-elements assuming that mixing occurs in the process of accretion (with mixing fraction 0.25). We present and contrast ignition mass, ejected mass, recurrence period and maximum luminosity of novae for different WD masses and accretion rates for these metallicities and mixing cases. We find that models with Z = 0.02 have ignition masses and recurrence periods smaller than models with low Z, while the ejected mass and maximum luminosity are larger. Retention efficiency during novae outbursts decreases with increasing metallicity. In our implementation, inclusion of mixing at the H/He interface reduces accreted mass, ejected mass and recurrence period as compared to the no-mixing case, while the maximum luminosity becomes larger. Retention efficiency is significantly reduced, becoming negative in most of our models. For ease of use, we provide a tabular summary of our results.

==> tables/SNBB_z1m4.tex <==
\begin{table}
\caption{Steady burning boundaries for $Z = 10^{-4}$. The first column is the WD mass; The second and third columns are the lower and upper boundaries, repectively.}
\label{tab:snbb_z1m4}
\begin{tabular}{ccc}
\hline
    \mwd\; (\msun) &        $\dot{M}_{\rm lower}(M_{\odot}/{\rm yr})$  &     $ \dot{M}_{\rm up}(M_{\odot}/{\rm yr})$\\
\hline
0.51   &         9.8e-9     &             5.12e-8\\ 
0.60   &         2.13e-8    &             9.36e-8\\  
0.70   &         4.1e-8     &             1.55e-7\\ 
0.80   &         6.0e-8     &             2.18e-7\\ 
0.90   &         8.2e-8     &             3.02e-7\\ 
1.00   &         1.07e-7    &             4.08e-7\\ 
1.10   &         1.39e-7    &             4.54e-7\\ 
1.20   &         1.74e-7    &             5.34e-7\\ 
1.30   &         2.42e-7    &             6.01e-7\\ 
\hline

\end{tabular}
\end{table}


==> tables/SNBB_z2m2.tex <==
\begin{table}
\caption{Steady burning boundaries for $Z = 0.02$. The first column is the WD mass; The second and third columns are the lower and upper boundaries, repectively.}
\label{tab:snbb_z2m2}
\begin{tabular}{ccc}
\hline
    \mwd\; (\msun)        &        $\dot{M}_{\rm lower}(M_{\odot}/{\rm yr})$  &     $ \dot{M}_{\rm up}(M_{\odot}/{\rm yr})$\\
\hline
0.51  &         0.25e-7    &            0.88e-7 \\
0.60  &         0.47e-7    &            1.42e-7 \\
0.70  &         0.73e-7    &            2.14e-7 \\
0.80  &         1.04e-7    &            2.86e-7 \\
0.90  &         1.37e-7    &            3.56e-7 \\
1.00  &         1.73e-7    &            4.26e-7 \\
1.10  &         2.19e-7    &            4.96e-7 \\  
1.20  &         2.65e-7    &            5.60e-7 \\
1.30  &         3.21e-7    &            6.24e-7 \\
\hline

\end{tabular}
\end{table}

